VcLLM: Video Codecs are Secretly Tensor Codecs

As the parameter size of large language models (LLMs) continues to expand, the need for a large memory footprint and high communication bandwidth have become significant bottlenecks for the training and inference of LLMs. To mitigate these bottlenecks, various tensor compression techniques have been proposed to reduce the data size, thereby alleviating memory requirements and communication pressure. Our research found that video codecs, despite being originally designed for compressing videos, show excellent efficiency when compressing various types of tensors. We demonstrate that video codecs can be versatile and general-purpose tensor codecs while achieving the state-of-the-art compression efficiency in various tasks. We further make use of the hardware video encoding and decoding module available on GPUs to create a framework capable of both inference and training with video codecs repurposed as tensor codecs. This greatly reduces the requirement for memory capacity and communication bandwidth, enabling training and inference of large models on consumer-grade GPUs.

==> src/dist_inference.tex <==
While our weight-only compression results show the ability of serving a 70B model on a single consumer-level GPU (i.e., about 24 GB of memory), it still suffers from two limitations in real-world applications. First, in long-context scenarios, we encounter issues with the size of the KV cache. For example, storing a 128k KV cache using FP16 requires 40 GB of GPU memory for LLaMA-3-70B, which is larger than the compressed model itself. Second, for on-device inference with only about 8 GB of memory, it is infeasible to efficiently run inference for a 70B model using a single edge device. To address these challenges, we aim to unlock the potential of distributed inference for LLMs in long-context, on-device settings. Specifically, we consider the extreme case of serving a 70B model with a 128k sequence length across four 8GB edge devices with pipeline parallelism. To address the challenges of limited memory capacity and communication overhead, we compress both the KV cache and activations.

\subsection{Experiments}
\label{sec:inference-experiment}

\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{figs/distributed_inference.pdf}
    \caption{\textbf{[Distributed Inference]:} The comparison between RTN and \name for compressing activations and KV cache of LLaMA-3-70B~\cite{llama3}. "KV3" represents compressing the KV Cache to 3 bits (2.9 bits for \name), while "A4" denotes compressing activations to 4 bits (3.5 bits for \name). Here we only compress activation for pipeline parallelism.}
    \label{fig:distributed_inference}
\end{figure}

Building on our compressed LLaMA-3-70B model in \autoref{sec:weight_only_exp}, we further compress the KV cache to 2.9 bits and the activations between different pipeline parallelism stages to 3.5 bits.   Similarly, we also first compress them to INT8 using channel-wise RTN quantization.  For baseline comparisons, since these values are runtime dynamics and cannot be preprocessed in advance, we employ RTN quantization to directly reduce the KV cache and activations to 3 bits and 4 bits, respectively, using asymmetric min-max dynamic quantization. Our evaluation includes measuring the perplexity score on the WikiText-2 testset and the zero-shot accuracy on the PIQA dataset.

As shown in \autoref{fig:distributed_inference}, our method results in only a 7\% increase (from 7.28 to 7.77) in perplexity score on wikitext2  and a 1\% drop (from 81.5\% to 80.7\%) in accuracy on PIQA while compressing the KV by 5.5 times and the activations by 4.5 times. Consequently, when the model is distributed across four devices using pipeline parallelism, only about 6.3 GB of memory is required for the compressed model and 1.8 GB for the stored KV cache. This totals approximately 8 GB of memory per device. Compared to RTN quantization, we observe that directly quantizing the KV cache to 3 bits leads to a significant performance drop, nearly destroying the original model's ability. For activation-only compression, our method achieves only a 5\% increase in perplexity score while RTN quantization results in a 13\% increase. Although this difference appears small and does not affect zero-shot accuracy on PIQA, it is important to note that we only compress the activation three times. Increasing the number of stages in pipeline parallelism will gradually widen this gap.


